Singular Perturbation of Zero-Sum Linear-Quadratic Stochastic Differential Games

We investigate a class of zero-sum linear-quadratic stochastic differential games on a finite time horizon governed by multiscale state equations. The multiscale nature of the problem can be leveraged to reformulate the associated generalised Riccati equation as a deterministic singular perturbation problem. In doing so, we show that, for small enough $\epsilon$, the existence of solution to the associated generalised Riccati equation is guaranteed by the existence of a solution to a decoupled pair of differential and algebraic Riccati equations with a reduced order of dimensionality. Furthermore, we are able to formulate a pair of asymptotic estimates to the value function of the game problem by constructing an approximate feedback strategy and observing the limiting value function.

==> packages.tex <==
%\usepackage{T1enc}

%\usepackage{multicol}    % used for the two-column index
\usepackage{upgreek}
%\usepackage{algorithmic}
%\usepackage[square]{natbib}
%\bibpunct[; ]{(}{)}{,}{a}{}{;} 
%\usepackage{a4}
\usepackage{wrapfig}
\usepackage{boxedminipage}
%\usepackage{boites} 
\usepackage{pifont}
%\usepackage{tweaklist}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{algmatlab}
\usepackage{euscript}
\usepackage{dcolumn}
%\usepackage{fancyheadings}
\usepackage{float}
\usepackage{fancybox}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{txfonts}
\usepackage{amsmath}
%\usepackage{amsthm}  % gives different style
\usepackage{epsfig}
\usepackage{color}
\usepackage{verbatim}
\usepackage{subfigure}
\usepackage{mathrsfs}
\usepackage{url}
\usepackage{lscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Post Script Font File(s)

% For TimesRoman Math (You must have MathTimes and MathTimes Plus 
%                        font sets, order fonts from  www.yandy.com)
% \usepackage[mtbold,noTS1]{m-times}

% For PostScript text
%\usepackage{w-bookps}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graphicx.sty for Including PostScript .eps files

%% If you don't have graphicx.sty available, unzip the graphics.zip
%% file included in this package.

% Choose one of these options, based on the system that you are using.
% If none look like your system, use dvips
% [dvips], [xdvi], [dvipdf], [dvipsone], [dviwindo], [emtex], [dviwin],
% [pctexps],  [pctexwin],  [pctexhp],  [pctex32], [truetex], [tcidvi],
% [oztex], [textures]

\usepackage{graphicx}

%\usepackage{hyperref} %Automatic hyperlinks in pdf.

